VL-Grasp: a 6-Dof Interactive Grasp Policy for Language-Oriented Objects in Cluttered Indoor Scenes

Robotic grasping faces new challenges in human-robot-interaction scenarios. We consider the task that the robot grasps a target object designated by human's language directives. The robot not only needs to locate a target based on vision-and-language information, but also needs to predict the reasonable grasp pose candidate at various views and postures. In this work, we propose a novel interactive grasp policy, named Visual-Lingual-Grasp (VL-Grasp), to grasp the target specified by human language. First, we build a new challenging visual grounding dataset to provide functional training data for robotic interactive perception in indoor environments. Second, we propose a 6-Dof interactive grasp policy combined with visual grounding and 6-Dof grasp pose detection to extend the universality of interactive grasping. Third, we design a grasp pose filter module to enhance the performance of the policy. Experiments demonstrate the effectiveness and extendibility of the VL-Grasp in real world. The VL-Grasp achieves a success rate of 72.5\% in different indoor scenes. The code and dataset is available at https://github.com/luyh20/VL-Grasp.

==> data_ana.tex <==
The average length of the expressios is 9.5, see Figure \ref{fig:sentence_len} for detailed distribution of sentence lengths. Our dataset contains objects of different sizes, which imposes requirements on the ability of the models to handle multi-scale targets. Figure \ref{fig:bbox_mask_size} shows the cumulative distribution curve of the size of bounding boxes and masks. For most of the images we select up to five targets for annotation, and in some images we select only some of the higher-quality targets for annotation, see Figure \ref{fig:bbox_pre_image} for detailed information. Figure \ref{fig:cloud} shows the words and phrases that frequently appear in expressions. Figure \ref{fig:cat} shows all the categories we use and the distribution of samples over them.

\begin{figure}
  \centering
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/sentence_len.png}
    \caption{Distribution of sentence lengths.}
    \label{fig:sentence_len}
  \end{minipage}
  \hspace{0.08\textwidth}
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/bbox_mask_size.png}
    \caption{Cumulative distribution of the size of bounding boxes and masks.}
    \label{fig:bbox_mask_size}
  \end{minipage}
\end{figure}

\begin{figure}
  \centering
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/target_per_img.png}
    \caption{Number of targets per image.}
    \label{fig:bbox_pre_image}
  \end{minipage}
  \hspace{0.05\textwidth}
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/wordcloud.png}
    \caption{Word cloud of RefIndoor dataset.}
    \label{fig:cloud}
  \end{minipage}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{imgs/cat.png}
  \caption{Number of samples per category.}
  \label{fig:cat}
\end{figure}
